GigaChat Family: Efficient Russian Language Modeling Through Mixture of Experts Architecture

Generative large language models (LLMs) have become crucial for modern NLP research and applications across various languages. However, the development of foundational models specifically tailored to the Russian language has been limited, primarily due to the significant computational resources required. This paper introduces the GigaChat family of Russian LLMs, available in various sizes, including base models and instruction-tuned versions. We provide a detailed report on the model architecture, pre-training process, and experiments to guide design choices. In addition, we evaluate their performance on Russian and English benchmarks and compare GigaChat with multilingual analogs. The paper presents a system demonstration of the top-performing models accessible via an API, a Telegram bot, and a Web interface. Furthermore, we have released three open GigaChat models in open-source (https://huggingface.co/ai-sage), aiming to expand NLP research opportunities and support the development of industrial solutions for the Russian language.

==> tables/en_benchs.tex <==
\begin{table*}[htp!]
\tiny
\begin{tabular}{
>{}l 
>{}l 
>{}l 
>{}l 
>{}l}
{\textbf{Bench}}  & { \textbf{T-lite-0.1}} & {\textbf{Llama-3.1-8B}} & { \textbf{\gigabase}} & {\textbf{Gemma-2-9B}} \\
\toprule
{ MMLU EN 5-shot}                                                           & { 62.56}               & { 65.21}                 & { 63.02}                          & { 70.6}                \\
{ MMLU PRO EN 5-shot}                                                       & { 32.19}               & { 35.7}                  & { 31.41}                          & { 42.85}               \\
{ MMLU RU 5-shot}                                                           & { 55.51}               & { 54.1}                  & { 58.38}                          & { 62.57}               \\
{ BBH 3-shot}                                                               & { 62.36}               & { 62.79}                 & { 53.54}                          & { 70.48}               \\
{ ARC-C 25-shot}                                                            & { 58.19}               & { 54.69}                 & { 61.69}                          & { 68.34}               \\
{ TruthfulQA 0-shot (rougeL)}                                               & { 46.51}               & { 34.52}                 & { 31.82}                          & { 41.49}               \\
{ Winogrande 5-shot}                                                        & { 78.45}               & { 77.43}                 & { 75.85}                          & { 79.4}                \\
{ Hellaswag 10-shot}                                                        & { 82.21}               & { 81.85}                 & { 81.91}                          & { 82.5}                \\
{ GPQA 5-shot}                                                              & { 25.0}                & { 23.44}                 & { 25.22}                          & { 30.36}               \\
{MATH 4-shot} & { 12.9}                & { 14.04}                 & { 15.04}                          & { 20.06}               \\
{GSM8K 4-shot } & { 67.93}               & { 51.4}                  & { 59.06}                          & { 68.99}               \\
{HumanEval}  & { 16.46}               & { 25.61}                 & { 32.32}                          & { 37.2}                \\
\midrule
{\textbf{AVG}}  & { 47.96}               & { 48.4}                  & { 49.11}                         & { 56.24} \\
\bottomrule
\end{tabular}
\end{table*}

% ЕЩЁ сюда надо IFEVAL

==> tables/hyperparams_example.tex <==
\begin{table}[h!]
\centering
    \small
    
\begin{tabular}{lcccc}
\toprule
 \textbf{Model} & \textbf{Optimizer} & \textbf{Learning Rate} &  \textbf{Weight Decay}  & \textbf{Batch Size} \\

\midrule
\multicolumn{5}{c}{\textbf{Russian SuperGLUE}} \\
\midrule
Encoder LMs & AdamW & $ 1\cdot10^{-5}$ & $0.01$ & $32$ \\
Decoder LMs & \xmark & \xmark  & \xmark & \xmark \\
Encoder-decoder LMs (I) &  Adafactor & $1\cdot10^{-3}$ & $15$ & $16$\\
Encoder-decoder LMs (II) & Adam & $1\cdot10^{-5}$ & $20$ & $16$\\

\midrule
\multicolumn{5}{c}{\textbf{RuCoLA}}\\
\midrule
ruBERT-base & AdamW & $3 \cdot 10^{-5}$ & $1e^{-4}$ & $64$ \\
ruBERT-large & AdamW & $3 \cdot 10^{-5}$ & $0.1$ & $64$ \\
ruBERT-base (DP) & AdamW  & $3 \cdot 10^{-5}$ & $0.01$ & $64$\\
ruBERT-base-conv (DP)  & AdamW & $1 \cdot 10^{-5}$ & $0.01$ & $32$ \\ 
mBERT  & AdamW & $1 \cdot 10^{-5}$ & $0.1$ & $32$  \\ 
ruRoBERTa-large & AdamW & $10^{-5}$ & $10^{-4}$ & $32$ \\
ruELECTRA-small & AdamW & $5 \cdot 10^{-5}$ & $0.1$ & $32$ \\
ruELECTRA-medium & AdamW & $5 \cdot 10^{-5}$ & $0.1$ & $32$ \\
ruELECTRA-large & AdamW & $3 \cdot 10^{-5}$ & $10^{-4}$ & $32$ \\
ruT5-base & Adafactor & $10^{-4}$ & $0$&  $128$ \\
ruT5-large & Adafactor & $10^{-4}$ & $0$&  $128$ \\
FRED-T5-large & Adafactor & $5 \cdot 10^{-4}$ & $0$&  $16$ \\
FRED-T5-XL & Adafactor & $5 \cdot 10^{-4}$ & $0$&  $16$
\\ 

\midrule
\multicolumn{5}{c}{\textbf{Inappropriateness Identification}}\\
\midrule
ruBERT-base & AdamW & $1 \cdot 10^{-5}$ & $0.1$ & $64$ \\
ruBERT-large & AdamW & $1 \cdot 10^{-5}$ & $0.1$ & $16$ \\
ruBERT-base (DP) & AdamW  & $1 \cdot 10^{-5}$ & $0.1$ & $64$\\
ruBERT-base-conv (DP)  & AdamW & $1 \cdot 10^{-5}$ & $0.01$ & $64$ \\ 
mBERT  & AdamW & $3 \cdot 10^{-5}$ & $0.01$ & $32$  \\ 
ruRoBERTa-large & AdamW & $10^{-5}$ & $10^{-4}$ & $32$ \\
ruELECTRA-small & AdamW & $5 \cdot 10^{-5}$ & $10^{-3}$ & $64$ \\
ruELECTRA-medium & AdamW & $5 \cdot 10^{-5}$ & $0.01$ & $64$ \\
ruELECTRA-large & AdamW &  &  &  \\
ruT5-base & Adafactor & $10^{-4}$ & $0$&  $128$ \\
ruT5-large & Adafactor & $10^{-4}$ & $0$&  $128$ \\
FRED-T5-large & Adafactor & $5 \cdot 10^{-4}$ & $0$&  $16$ \\
FRED-T5-XL & Adafactor & $5 \cdot 10^{-4}$ & $0$&  $16$

 \\ \midrule
\multicolumn{5}{c}{\textbf{Text Simplification}}\\
\midrule
Decoder LMs & AdamW & $1\cdot10^{-5}$ & $0$ & $2$ \\
Encoder-decoder LMs & AdamW & $1\cdot10^{-5}$ & $0$ & $2$ \\\midrule
\multicolumn{5}{c}{\textbf{Text Detoxification}}\\
\midrule
Decoder LMs & AdamW & $5 \cdot 10^{-5}$ & $0.01$ & $2$ \\
Encoder-decoder LMs & Adafactor & $1\cdot10^{-4}$ & $0.01$ & $8$ \\

\midrule
\multicolumn{5}{c}{\textbf{Text Summarization}}\\
\midrule
Decoder LMs & AdamW & $5 \cdot 10^{-5}$ & $0.01$ & $4$ \\
Encoder-decoder LMs & Adafactor & $1\cdot10^{-3}$ & $0.01$ & $2$ \\

\bottomrule
\end{tabular}
\caption{Optimal hyperparameter values found in the experiments. I/II=finetuning stage. DP=DeepPavlov~\cite{burtsev-etal-2018-deeppavlov}.}
\label{tab:hparams_finetune}
\end{table}

==> tables/posttraining_params.tex <==
\begin{table}[t!]
    \small
    \centering
    \setlength{\tabcolsep}{2pt}
    \begin{tabular}{lc}
    \toprule
    \textbf{Parameter} & \textbf{Value} \\
    \midrule
    Learning Rate & [5e-6, 5e-7] \\ 
    Global Batch Size & 320 \\ 
    Scheduler & Cosine or Constant with warmup \\ 
    Optimizer & Decoupled AdamW ($\beta = [0.9, 0.95]$, $\varepsilon=10^{-8}$) \\ 
    Gradient Clipping & $\lVert \nabla \rVert_{2} = 1$ \\ 
    \bottomrule
    \end{tabular}
    \caption{Training Hyperparameters}
    \label{tab:hyperparameters}
\end{table}


==> tables/time_speed.tex <==
\begin{table*}[h!]
\small
\begin{tabular}{
>{}l 
>{}l 
>{}l 
>{}l 
>{}l 
>{}l }
\toprule
\multicolumn{1}{c}{{\textbf{Model}}} & \multicolumn{1}{c}{{\textbf{Total params (B)}}} & \multicolumn{1}{c}{{\textbf{Active params (B)}}} & \multicolumn{1}{c}{{\textbf{Req/s}}} & \multicolumn{1}{c}{{\textbf{Output Token/s}}} & \multicolumn{1}{c}{{\textbf{Total Token/s}}} \\
\midrule
{Qwen/Qwen1.5-MoE-A2.7B-Chat}                                & {14}  & {2,7}   & {0,62}  & {156,43}  & {291,17}  \\
{deepseek-ai/deepseek-moe-16b-chat}            & {16}   & {2,8} & {0,59} & {149,53}   & {285,39}   \\
{\textbf{\gigainstruct}}                                  & {20}  & {3,3}  & {0,55}  & {137,43}  & {259,27}  \\
{Qwen/Qwen2.5-3B-Instruct}                                   & {3}  & {3}  & {0,54}  & {135,10}  & {251,44}  \\
{meta-llama/Meta-Llama-3-8B-Instruct}                        & {8}  & {8} & {0,35}   & {83,26} & {157,32}   \\
{google/gemma-2-9b-it}                                       & {9} & {9} & {0,27} & {54,87} & {113,69}          \\          \bottomrule
\end{tabular}
\caption{Speed assessments on the similar architectures.}
\end{table*}
